Efficient Learning of Fast Inverse Kinematics with Collision Avoidance

Fast inverse kinematics (IK) is a central component in robotic motion planning. For complex robots, IK methods are often based on root search and non-linear optimization algorithms. These algorithms can be massively sped up using a neural network to predict a good initial guess, which can then be refined in a few numerical iterations. Besides previous work on learning-based IK, we present a learning approach for the fundamentally more complex problem of IK with collision avoidance. We do this in diverse and previously unseen environments. From a detailed analysis of the IK learning problem, we derive a network and unsupervised learning architecture that removes the need for a sample data generation step. Using the trained network's prediction as an initial guess for a two-stage Jacobian-based solver allows for fast and accurate computation of the collision-free IK. For the humanoid robot, Agile Justin (19 DoF), the collision-free IK is solved in less than 10 milliseconds (on a single CPU core) and with an accuracy of 10^-4 m and 10^-3 rad based on a high-resolution world model generated from the robot's integrated 3D sensor. Our method massively outperforms a random multi-start baseline in a benchmark with the 19 DoF humanoid and challenging 3D environments. It requires ten times less training time than a supervised training method while achieving comparable results.

==> tables/ablation_study_network.tex <==
\begin{tabular}{ccc|cccccccc}
\toprule
            &                &         & \multicolumn{2}{c}{Position Error} & \multicolumn{2}{c}{Orientation Error } & \multicolumn{2}{c}{Obstacle Collision}  & \multicolumn{2}{c}{Self Collision}   \\
Training w. & Twin-Headed    & Unit Vector   & \multicolumn{2}{c}{$\CostFramePos$ [m]} & \multicolumn{2}{c}{$\CostFrameRot$ [rad]}        & \multicolumn{2}{c}{$\CostWorldCollision$ [mm]} & \multicolumn{2}{c}{$\CostSelfCollision$ [mm]} \\
Boosting    & Network        & Output  & mean   & max                       & mean   & max                           & mean  & max                            & mean  & max                           \\
\midrule
No     & No      & No      & 0.198  & 1.433                     & 0.198  & 3.073                         & 2.13  & 1260.10                        & 0.65  & 272.37                       \\
No     & No      & Yes     & 0.102  & 1.122                     & 0.081  & 2.338                         & 0.82  & 705.83                         & 0.38  & 128.32                       \\
No     & Yes     & No      & 0.152  & 1.079                     & 0.100  & 1.698                         & 0.55  & 700.29                         & 0.26  & 72.37                        \\
No     & Yes     & Yes     & 0.099  & 0.737                     & 0.067  & 1.312                         & 0.41  & 760.07                         & 0.51  & 70.43                        \\
Yes    & No      & No      & 0.208  & 1.033                     & 0.196  & 3.096                         & 2.38  & 927.62                         & 0.96  & 666.52                       \\
Yes    & No      & Yes     & 0.118  & 0.893                     & 0.116  & 3.125                         & 1.10  & 661.09                         & 0.47  & 251.48                       \\
Yes    & Yes     & No      & 0.174  & 0.797                     & 0.101  & 1.724                         & 0.57  & 576.50                         & 0.30  & 85.11                        \\
Yes    & Yes     & Yes     & 0.108  & 0.696                     & 0.087  & 0.981                         & 0.32  & 444.35                         & 0.09  & 59.05                        \\
\bottomrule
\end{tabular}
